N-Shot Benchmarking of Whisper on Diverse Arabic Speech Recognition

Whisper, the recently developed multilingual weakly supervised model, is reported to perform well on multiple speech recognition benchmarks in both monolingual and multilingual settings. However, it is not clear how Whisper would fare under diverse conditions even on languages it was evaluated on such as Arabic. In this work, we address this gap by comprehensively evaluating Whisper on several varieties of Arabic speech for the ASR task. Our evaluation covers most publicly available Arabic speech data and is performed under n-shot (zero-, few-, and full) finetuning. We also investigate the robustness of Whisper under completely novel conditions, such as in dialect-accented standard Arabic and in unseen dialects for which we develop evaluation data. Our experiments show that although Whisper zero-shot outperforms fully finetuned XLS-R models on all datasets, its performance deteriorates significantly in the zero-shot setting for five unseen dialects (i.e., Algeria, Jordan, Palestine, UAE, and Yemen).

==> Sections/preprocessing.tex <==

Some of the datasets we use have inconsistencies. For example, in CV6.1 the utterance \RL{فَقَالَ لَهُمْ} (faqaAla lahumo) has complete diacritic markings, while the utterance \RL{فإذا النجوم طمست} (f$<$*A Alnjwm Tmst) does not have any diacritics, even though both come from the Quran. For this reason, we follow~\cite{chowdhury2021towards} in standardizing the data. Namely, we (a) remove all punctuation except the \% and @ symbols; (b) remove diacritics, Hamzas, and Maddas; and (c) transliterate all eastern Arabic numerals to western Arabic numerals (e.g. \RL{٩٢} to 29). Since we do not treat code-switching in this work, we remove all Latin characters.
